Lithium NLP: A System for Rich Information Extraction from Noisy User Generated Text on Social Media

In this paper, we describe the Lithium Natural Language Processing (NLP) system - a resource-constrained, high- throughput and language-agnostic system for information extraction from noisy user generated text on social media. Lithium NLP extracts a rich set of information including entities, topics, hashtags and sentiment from text. We discuss several real world applications of the system currently incorporated in Lithium products. We also compare our system with existing commercial and academic NLP systems in terms of performance, information extracted and languages supported. We show that Lithium NLP is at par with and in some cases, outperforms state- of-the-art commercial NLP systems.

==> papyrus paper latex/texfiles/abstract.tex <==
%The Entity Disambiguation and Linking (EDL) task matches \emph{entity mentions} in text to a unique Knowledge Base (KB) identifier such as a Wikipedia or Freebase id. It plays a critical role in the construction of a high quality information network, and can be further leveraged for a variety of information retrieval and NLP tasks such as text categorization and document tagging. EDL is a complex and challenging problem due to ambiguity of the mentions and real world text being multi-lingual. Moreover, EDL systems need to have high throughput and should be lightweight in order to scale to large datasets and run on off-the-shelf machines. More importantly, these systems need to be able to extract and disambiguate dense annotations from the data in order to enable an Information Retrieval or Extraction task running on the data to be more efficient and accurate. In order to address all these challenges, we present the Lithium EDL system and algorithm - a high-throughput, lightweight, language-agnostic EDL system that extracts and correctly disambiguates 75\% more entities than state-of-the-art EDL systems and is significantly faster than them.
%%Our experiments demonstrate that our EDL system recognizes and disambiguates about 70\% more entities than the existing systems. 

In this paper, we describe the Lithium Natural Language Processing (NLP) system - a resource-constrained, high-throughput and language-agnostic system for  information extraction from noisy user generated text on social media. Lithium NLP extracts a rich set of information including entities, topics, hashtags and sentiment from text. We discuss several real world applications of the system currently incorporated in Lithium products. We also compare our system with existing commercial and academic NLP systems in terms of performance, information extracted and languages supported. We show that Lithium NLP is at par with and in some cases, outperforms state-of-the-art commercial NLP systems.

==> papyrus paper latex/texfiles/acknowledgements.tex <==
The authors would like to thank Prantik Bhattacharya, Adithya Rao and Sarah Ellinger for their contributions to the Lithium NLP system. They would also like to thank Mike Ottinger and Armin Broubakarian for their help with building the Lithium NLP UI and demo.

==> papyrus paper latex/texfiles/algorithm.tex <==
%\begin{algorithm*}[t]
%    \SetAlgoLined
%\KwInput{Text $T_{i}$ with extracted mentions $\mathbb{M}_{all}$ and a set of candidate entities for each mention}
%\KwOutput{Text $T_{i}$ with extracted mentions $\mathbb{M}_{all}$ and a unique disambiguated entity for each mention}
%\tcp{First pass - Disambiguate the easy mentions}
%$\mathbb{M}_{easy}$ $\leftarrow$ Easy mentions obtained from the first pass on $T_{i}$\;
%    $\mathbb{E}_{easy}$ $\leftarrow$ Disambiguated easy entities obtained from the first pass on $T_{i}$\;
%    Document Context $C(T_{i})$  $\leftarrow$ $C(T_{i})$ + $\mathbb{E}_{easy}$ \; 
%    $\mathbb{M}_{hard}$ $\leftarrow$ $\mathbb{M}_{all}$ - $\mathbb{M}_{easy}$\;
%    \tcp{Second pass - Iterate over the hard mentions}
%    \ForEach{Mention \emph{$M_{j}$} $\in$ $\mathbb{M}_{hard}$} {
%    $\mathbb{H}_{j}$ $\leftarrow$ Candidate entities of $M_{j}$\;
%    \tcp{Iterate over the candidate entities of a hard mention}
%    \ForEach{Entity \emph{$E_{k}$} $\in$ $\mathbb{H}_{j}$} {
%    Entity Context  C'($E_{k}$) $\leftarrow$ C'($E_{k}$) + $\mathbb{E}'_{k}$ (set of easy entities in a window around $E_{k}$) \;
%	$F_{E_{k}}$ $\leftarrow$ Generate feature vector of context independent and dependent features values for $E_{k}$ using C'($E_{k}$)\;
%	Classify $F_{E_{k}}$ as one of \emph{$\left\{\text{True, False}\right\}$} using Decision Tree classifier\;
%	$S_{E_{k}}$ $\leftarrow$ Final score for $E_{k}$ generated using Logistic Regression model weights\;
%	Add $S_{E_{k}}$ to set $S_{j}$ (Set of candidate entity scores for \emph{$M_{j}$})\;
%    }
%    \tcp{Final disambiguation - select one of the candidate entities as disambiguated entity $D_{j}$ for \emph{$M_{j}$}}
%    	\uIf{Only one $E_{k}$ $\in$ $\mathbb{H}_{j}$ labeled as  \emph{True}} {
%	 	$D_{j}$ $\leftarrow$ $E_{k}$ labeled as \emph{True}\;
%	}  \uElse {
%	\uIf{Multiple $E_{k}$ labeled as True}{
%		$D_{j}$ $\leftarrow$ Highest scoring $E_{k}$ labeled as \emph{True}\;
%	}  \uElseIf{None of $E_{k}$ labeled as True}{
%		$D_{j}$ $\leftarrow$ $\argmax$ ($S_{E_{k}}$)\;
%	}
%	\uIf{$D_{j}$ is \textbf{NIL} and \emph{NIL\_MARGIN\_GAIN} < threshold} {
%		$D_{j}$ $\leftarrow$ $\argmax$ ($S_{j}$ - $S_{D_{j}}$)\;
%	}
%}
%}
%    \Return{Text with extracted mentions and disambiguated entities\;}
%      \caption{Lithium EDL algorithm}
%    \label{alg:nedl}
%\end{algorithm*}

%As mentioned earlier, the Lithium EDL system uses a two pass algorithm for disambiguating and linking entities. 

Algorithm \ref{alg:nedl} describes the Lithium EDL two-pass algorithm. %In the first pass, we disambiguate easy entities while in the second pass, we utilize the easy entities within a given window to disambiguate hard entities. 
We discuss it in detail now (the design choices for various parameters are explained in Section \ref{section:tuning}).

\subsection{First pass \label{firstpass}}
The first pass of the algorithm iterates over all mentions in the document text and disambiguates mentions that have:
\begin{itemize}[noitemsep,nolistsep]
\item Only one candidate entity: In this case, the algorithm disambiguates the mention to the lone candidate entity.
\item Two candidate entities with one being \textbf{NIL}/\textbf{MISC}:  In this case, the algorithm disambiguates the mention to the candidate entity with high \emph{Mention-Entity-Cooccurr} prior probability (above $\lambda_{1}$ - Easy Mention Disambiguation threshold with \textbf{NIL}).
%Based on our experiments on a validation set (which consists of 10 Wikipedia pages generated using the process described in Section \ref{data_set}), we set this confidence threshold as 0.75.
\item Three or more candidate entities with one entity mapping with very high prior: In this case, the algorithm disambiguates the mention to the candidate entity with high \emph{Mention-Entity-Cooccurr} prior probability (above $\lambda_{2}$ - Easy Mention Disambiguation threshold). 
%Based on experiments on the validation set, we set the confidence threshold as 0.9. 

\end{itemize}

Mentions disambiguated in the first pass constitute the set $\mathbb{M}_{easy}$ and their corresponding disambiguated entities constitute the set $\mathbb{E}_{easy}$. The remaining ambiguous mentions constitute the set $\mathbb{M}_{hard}$ and are disambiguated in the second pass.

\subsection{Second pass}
The second pass of the algorithm uses several context-independent and context-dependent features as well as supervised classifiers to label and score the candidate entities for each hard mention and finally disambiguate it. 

\subsubsection{\textbf{Features}} \label{sec:features}

We use several language agnostic features to classify each candidate entity for each hard mention as `True' or `False'. These include both context-independent (useful for disambiguating and linking entities in short and sparse texts such as tweets) as well as context-dependent features (useful for disambiguating and linking entities in long and rich text). Each feature produces a real value in [0.0,1.0].

The context independent features are:

\begin{itemize}[noitemsep,nolistsep]

\item \textbf{Mention-Entity Cooccurrence} (\emph{Mention-Entity-Cooccurr}) - This feature value is equal to the \emph{Mention-Entity-Cooccurr} prior probability.

\item \textbf{Mention-Entity Jaccard Similarity} (\emph{Mention-Entity-Jaccard}) - This reflects the similarity between the mention $M_{i}$ and the representative name of a candidate entity $E_{j}$. The mention and the entity display names are first tokenized and the Jaccard similarity is then computed between the token sets as
%Can we describe why this feature is useful or what are the additional information this feature tries to capture?
\small
$$
%\emph{Mention-Entity-Jaccard} = {{Tokens(M_{i}) \cap Tokens(E_{j})} \over {Tokens(M_{i}) \cup Tokens(E_{j})}}
{{Tokens(M_{i}) \cap Tokens(E_{j})} \over {Tokens(M_{i}) \cup Tokens(E_{j})}}
$$
%This feature produces a real value in [0.0,1.0].
\normalsize
For instance, the mention \emph{Marvel} could refer to the entities \emph{Marvel Comics} or \emph{Marvel Entertainment}, both of which have a Jaccard Similarity of 0.5 with the mention.

\item \textbf{Entity Importance} (\emph{Entity-Importance}) - This reflects the importance or the relevance of the candidate entity as determined by an entity scoring and ranking algorithm \cite{Bhattacharyya-importance} which ranks the top 1 million entities occurring in our KB. For instance, the entity \emph{Apple Inc.} has an importance of 0.66 while \emph{Apple (fruit)} has an importance of 0.64 as ranked by the Entity Scoring algorithm.

\end{itemize}

\begin{figure}[t]
\centering
\includegraphics[width=75mm ,height=35mm]{figures/TopicOntologySemanticDistance.pdf}
\vspace{-0.1in}
\caption{Semantic distance between topics in Klout Topic Ontology Space}
\label{fig:topicsimdist}
\vspace{-0.1in}
\end{figure}

For the following context dependent features, we assume that for a candidate entity $E_{i}$, we maintain an entity context C'($E_{i}$) which contains a window $\mathbb{E}'_{i}$ of \emph{W} disambiguated easy entities immediately surrounding $E_{i}$.

\begin{itemize}[noitemsep,nolistsep]
\item \textbf{Entity Entity Cooccurrence} (\emph{Entity-Entity-Cooccurr}) - 
%The entity context for each hard mention in the text
%, as computed after the First Pass of our algorithm (Section \ref{firstpass}), includes the easy mentions that have been disambiguated in the immediate window of the hard mention. 
This feature value is equal to the averaged co-occurrence of a candidate entity with the disambiguated easy entities in $\mathbb{E}'_{i}$ and is computed as:
%For instance, for a candidate entity $E_{i}$ and the set $\mathbb{E}'_{i}$ of easy entities in $E_{i}$'s window, the feature is computed as:
\small
%\emph{Entity-Entity-Cooccurr}  = 
$$
{\sum_{j=1}^{W} Co-occurrence-count (E_{i}, E_{j}) \over {W}} \forall E_{j} \in  \mathbb{E}'_{i}
$$
%This feature produces a real value in [0.0,1.0].
\normalsize

\item \textbf{Entity Entity Topic Semantic Similarity} (\emph{Entity-Entity-Topic-Sim}) - As mentioned in Section \ref{subsection:OfflineDictionary}, each entity in our KB is associated with a finite number of topics in our topic ontology. For instance, entity \emph{Apple Inc.} maps to the topic `Apple' and \emph{Google Inc.} maps to the topic `Google' while `\emph{Apple (fruit)}' will map to the topic `Food'. Figure \ref{fig:topicsimdist} shows a partial view of the ontology for the above mentioned topics.  
%A complete description of the Topic Ontology is beyond the scope of this paper.

For each candidate entity $E_{i}$ of a hard mention $M_{i}$, we compute the minimum \emph{semantic distance} of its topics with topics of each entity in $\mathbb{E}'_{i}$ over all possible paths in our topic ontology space. The similarity is the inverse of the distance. For instance, consider the hard mention \emph{Apple}, having two candidate entities - \emph{Apple Inc.} and \emph{Apple (fruit)} for it, and $\mathbb{E}'_{i}$ containing the entity \emph{Google Inc.} which has been disambiguated. As shown in Figure \ref{fig:topicsimdist}, the semantic distance between the topics for \emph{Apple Inc.} and \emph{Google Inc.} is 4 while the semantic distance between the topics for \emph{Apple (fruit)} and \emph{Google Inc.} is 5. As a result, it is more likely that \emph{Apple} disambiguates to \emph{Apple Inc}. 

Thus, we first determine the set of topics $\mathbb{T}_{i}$ that the candidate entity $E_{i}$ is associated with. For each entity $E_{j}$ in $\mathbb{E}'_{i}$, we generate the set of topics $\mathbb{T}_{j}$. The feature value is computed as
\small
$$
\max {1 \over distance (t_{i}, t_{j})} \forall t_{i} \in \mathbb{T}_{i}, t_{j} \in \mathbb{T}_{j}
$$
\normalsize
\end{itemize}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth,height=80mm]{figures/RunningExample.pdf}
\vspace{-0.3in}
\caption{Disambiguation of a sample sentence (best viewed in color)}
\label{fig:sample}
 \vspace{-0.1in}
\end{figure*}

\subsubsection{\textbf{Classification and Scoring}}

As a penultimate step in the second pass, the computed features are combined into a feature vector for a candidate entity and the Decision Tree classifier labels the feature vector as `True' or `False'. In addition, for each candidate entity, we also generate final scores using weights generated by the Logistic Regression classifier that we trained in Section \ref{subsubsec:class}. We use an ensemble of the two classifiers in the final disambiguation step as it helps overcome the individual bias of each classifier.
%Needs to explain why we are not using the score from Decision Tree.

\subsubsection{\textbf{Final Disambiguation}}
The final disambiguation step needs to select one of the labeled candidate entities as the disambiguated entity for the mention. However, multiple cases arise at the time of disambiguation:
\begin{itemize}[noitemsep,nolistsep]
\item Only one candidate entity is labeled as `True'- Here, the algorithm selects that entity as the disambiguated entity for the given mention.
\item Multiple candidate entities labeled  as `True'  - Here, the algorithm selects the highest scoring entity (from among those labeled `True') as the disambiguated entity except when this entity is \textbf{NIL}/\textbf{MISC}. In that case, the algorithm checks the \emph{margin of gain} or the score difference between the \textbf{NIL}/\textbf{MISC} entity and the next highest scoring entity that is labeled `True'. If the margin of gain is less than a threshold (less than \textbf{NIL} margin of gain threshold, $\lambda_{3}$) then the next highest scoring entity (from among those labeled `True') is selected.
\item All candidate entities labeled as `False' - Here, the algorithm selects the highest scoring entity as the disambiguated entity except when this entity is \textbf{NIL}/\textbf{MISC}. In that case, the algorithm checks the margin of gain for this entity over the next highest scoring entity. If the margin of gain is less than a threshold (less than \textbf{NIL} margin of gain threshold, $\lambda_{3}$) then the next highest scoring entity is selected.
\end{itemize}
%Based on our experiments on the validation set, we set the \emph{margin of gain} as 0.5

\subsection{Demonstrative Example}\label{sec:demoex}

To demonstrate the efficacy of our algorithm, let's disambiguate the sample text: 
\emph{``Google CEO Eric Schmidt said that the competition between Apple and Google and iOS vs.  Android is `the defining fight of the tech industry.' ".} 

Figure \ref{fig:sample} walks through the disambiguation of the sample text. The Text Preprocessing stages extract the mentions (highlighted in bold) and generate the candidate entities and the prior cooccurrence scores for each mention\footnote{Though our algorithm utilizes the Freebase machine id for each candidate entity, we only show the entity name for clarity.}. 
As shown, the extracted mentions and their candidate entities are:
\begin{itemize}[noitemsep,nolistsep]
\item \emph{Google} - \textbf{NIL} and \emph{Google Inc.}
\item \emph{CEO} - \textbf{NIL} and \emph{Chief Executive}
\item \emph{Eric Schmidt} - \textbf{NIL} and \emph{Eric Schmidt}
\item \emph{Apple} - \textbf{NIL}, \emph{Apple (fruit)}, \emph{Apple Inc.} and \emph{Apple Records}
\item \emph{iOS} - \textbf{NIL} and \emph{iOS}
\item \emph{Android} - \textbf{NIL}, \emph{Android (OS)} and \emph{Android(robot)}
\item \emph{tech industry} - \emph{Technology}
\end{itemize}
In the first pass, the algorithm disambiguates the easy mentions. Based on their high prior scores and number of candidate entities, it disambiguates \emph{Eric Schmidt}, \emph{iOS} and \emph{tech industry} (highlighted in color) to their correct entities. 
In the second pass, it uses the easy mention window and computes several context dependent and independent features to score and classify the candidate entities of the hard mentions. Note that for the purpose of clarity and simplicity, we are not walking through the feature and final score computation. As shown, for the remaining hard entities, it has classified the candidate entities as `True' or `False'.
In the final disambiguation step, it selects one of the labeled entities as the correct disambiguated entity. In the sample sentence, for all the mentions, only one of the candidate entities is labeled as `True', and hence the algorithm selects that entity  as the disambiguated entity for each mention.

%Its quite evident that our EDL system can recognize several entities mentioned in the text and utilize this rich annotated content to understand the topics or the categories the text is about as well as 



==> papyrus paper latex/texfiles/applications.tex <==
\begin{figure*}[t]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/ExpertiseScore.png}
    \caption{Topics of expertise a User }
            \vspace{-0.1in}
    \label{fig:expertise_score}
  \end{minipage}
  \qquad
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/ContentDiscovery.png}
    \caption{Content Personalization}
                \vspace{-0.1in}
    \label{fig:content_discovery}
  \end{minipage}
 % \vspace{-0.1in}
\end{figure*}

As mentioned earlier, the Lithium NLP system is currently incorporated in several Lithium products including Klout, Lithium Reach and Response. Its applications include:

\begin{itemize}[nolistsep,noitemsep]
\item \textbf {User modeling} - Building topical profiles of users on Klout to model their interests and expertise.  An example of user expertise topics is shown in Figure \ref{fig:expertise_score}. Currently, we build topical profiles for more than 600M users which are also available via GNIP PowerTrack\footnote{\url{http://support.gnip.com/enrichments/klout.html}}.
%We derive \textbf{topic profiles} of individual users by analyzing their social media texts and URLs with the pipeline. A profile contains two types of topics 

%\begin{itemize}[noitemsep, nolistsep]
%  \item Topics that are interesting to the user \cite{nemanja-lasta} 
%  \item Topics on which the user is an expert \cite{Spasojevic2016:experts}
%\end{itemize}
\item \textbf {Content Personalization} - We apply these topic profiles to recommend content to users by matching user and content topics as this leads to better user engagements. An example of content personalization on a Lithium product is shown in Figure \ref{fig:content_discovery}. %This tool is integrated into \url{https://klout.com} and \url{https://www.lithium.com/products/social-media-management/} 

\item \textbf{User Targeting} - This involves selecting a group of users for targeting based on given topics and other filtering criteria. Over the course of time, a version of Lithium NLP had been used to enable targeting applications such as Klout Perks\footnote{\url{https://goo.gl/vtZDqE\#Klout_Perks}} (influencer reward platform), Cinch\footnote{\url{https://goo.gl/CLcx9p\#Cinch}} (Q\&A app), and Who-To-Follow recommendations.

\end{itemize}


==> papyrus paper latex/texfiles/conclusion.tex <==
%In this paper, we presented the Lithium EDL system that disambiguates and links entity mentions in text to their unique Freebase ids. Our EDL algorithm uses several context dependent and context independent features to disambiguate mentions to their respective entities. Moreover, it recognizes several types of entities in addition to named entities like people, places, organizations. 
%In addition, our EDL system is language-agnostic and currently supports several languages including English, Arabic, Spanish, French, German, and Japanese. As a result, it is highly applicable to process real world text such as multi-lingual user generated content from social media in order to model user interests and expertise. 
%
%We compared our EDL system with several state-of-the-art systems and demonstrate that it has high throughput and is very lightweight. It can be run on an off-the-shelf commodity machine and scales easily to large datasets. Also, our experiments show that our EDL system extracts and correctly disambiguates about 75\% more entities than existing state-of-the-art commercial systems such as Google NLP Cloud API and Open Calais and is significantly faster than some of them.
%In future, we plan to add support for several other languages to our EDL system once we have collected enough ground truth data for them. We also plan to migrate to Wikipedia as our KB. We will also compare our system's performance against several state-of-the-art systems on metrics such as precision, recall and f-score with respect to existing benchmarked datasets.

In this paper, we described the Lithium NLP system - a resource-constrained, high-throughput and language-agnostic system for information extraction from noisy user generated text on social media. Lithium NLP extracts a rich set of information including entities, topics, hashtags and sentiment from text. We discussed several real world applications of the system currently incorporated in Lithium products. We also compared our system with existing commercial and academic NLP systems in terms of performance, information extracted and languages supported. We showed that Lithium NLP is at par with and in some cases, outperforms state-of-the-art commercial NLP systems.

In future, we plan to extend the capabilities of Lithium NLP to include entity level sentiment as well. We also hope to collaborate actively with academia and open up the Lithium NLP API to academic institutions.

==> papyrus paper latex/texfiles/dataset.tex <==
Since our goal is to build a language-agnostic NLP system, we needed a dataset that scales across several languages and also has good annotation density and coverage. Unfortunately, such a dataset is not readily available. 
Hence, we generated a ground truth data set for our NLP system, the Densely Annotated Wikipedia Text (DAWT) \cite{Spasojevic:dawt}, 
%used for derivation of the offline dictionaries and training data was based on
using densely Wikified \cite{Mihalcea:2007:WLD:1321440.1321475} or annotated Wikipedia articles. 
Wikification is entity linking with Wikipedia as the KB. We started with Wikipedia data dumps\footnote{\url{https://dumps.wikimedia.org/}},
which were further enriched by introducing more hyperlinks in the existing document structure. 
Our main goals when building this data set were to maintain high precision and increase linking coverage. 
As a last step, the hyperlinks to Wikipedia articles in a specific language were replaced with links to their Freebase ids to adapt to our KB. The densely annotated Wikipedia articles had on an average 4.8 times more links than the original articles.

==> papyrus paper latex/texfiles/evaluation.tex <==
%\begin{table}[t]
%\centering
%\begin{tabular}{|c|c|c|}
%\hline
% & \multicolumn{2}{|c|}{\textbf{Ground Truth Label}}  \\
% \cline{2-3}
%\textbf{Predicted Label}  & Correct Entity & \textbf{NIL} \\
%\hline
%  Correct Entity &TP & FP\\
%\hline
% Wrong Entity& FP & FP\\
%\hline
% \textbf{NIL} & FN & TN\\
%\hline
%\end{tabular}
%%\vspace{-0.1in}
%\caption{Confusion matrix for our EDL system}
%\label{PositivesNegatives}
%\vspace{-0.3in}
%\end{table}

%\begin{table*}[!th]
%\centering
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\textbf{Features} & \textbf{Precision} & \textbf{Recall} & \textbf{Accuracy} & \textbf{F-score}\\
%\hline
% \emph{Mention-Entity-Cooccurr} (context independent) & 0.65 & 0.75 & 0.70 & 0.62\\
%\hline
%\emph{Mention-Entity-Jaccard} (context independent) & 0.47 & 0.93 & 0.48 & 0.63\\
% \hline
%\emph{Entity-Importance} (context independent) & 0.50 & 0.90 & 0.50 & 0.65\\
% \hline
%\emph{Entity-Entity-Cooccurr} (context dependent) & 0.54 & 0.91 & 0.54 & 0.68\\
% \hline
%\emph{Entity-Entity-Topic-Sim} (context dependent) & 0.49 & 0.88 & 0.49 & 0.63\\
% \hline
%Combined Context independent features & 0.63 & 0.83 & 0.62 & 0.72\\
%  \hline
%Combined Context dependent features & 0.52 & 0.92 & 0.52 &0.66\\
%\hline
%All features & 0.63 & 0.87 &  0.64 & 0.73\\
%\hline
%\end{tabular}
%%\vspace{-0.1in}
%\caption{Precision, recall, accuracy, and f-score for different features and feature sets on our test set (English only)}
%\label{FeatureEffectiveness}
%\vspace{-0.2in}
%\end{table*}
%
%\begin{table}[!th]
%\centering
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\textbf{Language} & \textbf{Precision} & \textbf{Recall} & \textbf{F-score} & \textbf{Accuracy}\\
%\hline
%English & 0.63 & 0.87 & 0.73 & 0.64\\
%\hline
%French & 0.59 & 0.86 & 0.70 & 0.6\\
% \hline
%German & 0.63 & 0.90 & 0.74 & 0.64\\
% \hline
%Spanish & 0.58 & 0.89 & 0.70 & 0.60\\
% \hline
%Japanese & 0.73 & 0.88 & 0.80 & 0.74\\
% \hline
% \end{tabular}
%% \vspace{-0.1in}
%\caption{Precision, recall, f-score and accuracy across various languages}
%\label{LanguagePerf}
%\vspace{-0.3in}
%\end{table}

%\begin{minipage}[b]{1\linewidth} 
%\centering
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\textbf{Algorithm} & \textbf{Precision} & \textbf{Recall} & \textbf{F-score} & \textbf{Accuracy}\\
%\hline
%Baseline Disambiguation and Linking algorithm & 0.55 & 0.99 & 0.7 & 0.62\\
%\hline
%Context-driven Entity Disambiguation and Linking algorithm  & 0.63 & 0.87 & 0.73 & 0.64\\
%\hline
%\end{tabular}
%\caption{Precision, Recall, F-score and Accuracy for our algorithm and baseline (English only)}
%\label{baselinecomparison}
%\end{minipage}
%\end{table*}

%\begin{figure}[t]
%  \centering
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=\textwidth,height=55mm]{figure/papyrus_performance_per_language_per_stage/eps/en_performance.eps}
%    \caption{Processing Stages for English}
%    \label{fig:processing_times_per_stage}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=\textwidth,height=55mm]{figure/papyrus_performance_per_language_per_stage/eps/ENTITY_DISAMBIGUATION_performance.eps}
%    \caption{Different Languages for Entity Disambiguation}
%    \label{fig:processing_times_per_language}
%  \end{subfigure}
%    \vspace{-0.1in}
%  \caption{Processing times as function of text length}
%  \label{fig:processing_times}
%  \vspace{-0.2in}
%\end{figure}

\subsection{Test datasets}
Using the process described in Section \ref{data_set}, we generated a ground truth test set of 20 English Wikipedia pages which had a total of 18,773 mentions. %We use this as our test set.

\subsection{Metrics}
We use standard performance metrics like precision, recall, f-score and accuracy to evaluate our NLP system components on the test sets. %However, due to our problem setup, we calculate true positives, false positives, and true negatives and false negatives in an unconventional way as shown in Table \ref{PositivesNegatives}. 
Precision, recall, f-score and accuracy are calculated as:
 $
 \textnormal{P} = {{\textnormal{$t_{p}$}} \over {\textnormal{$t_{p} $+ $f_{p}$}}}
$,
$
 \textnormal{R}= {{\textnormal{$t_{p}$}} \over {\textnormal{$t_{p}$ + $f_{n}$}}}
$,
$
 \textnormal{F1}= {{2 \times \textnormal{P} \times \textnormal{R}} \over {\textnormal{P + R}}}
$
and 
$
 \textnormal{Accuracy} = {{\textnormal{$t_{p}$ + $t_{n} $}} \over {\textnormal{$t_{p}$ + $t_{n}$ + $f_{p}$ + $f_{n}$}}}
$

\subsection{Results}\label{sec:results}
%Discussion about the features and results
%We compute the performance metrics for individual features as well as for various feature sets on our English language test set to assess their impact. % of individual features as well as feature sets. 
%Table \ref{FeatureEffectiveness} shows the feature effectiveness results for our algorithm. As evident from the results, \emph{Mention-Entity-Cooccurr} has the biggest impact on the performance of the algorithm among all individual features as it has the highest individual precision and f-score. %among all individual features. 
%
%When combined, the context independent features combined %(\emph{Mention-Entity-Cooccurr}, \emph{Mention-Entity-Jaccard} and \emph{Entity-Importance}) 
%have higher precision and f-score than the context dependent features. %(\emph{Entity-Entity-Cooccurr} and \emph{Entity-Entity-Topic-Sim}). 
%This could be due to the fact that in shorter text documents, there may not be enough easy mentions disambiguated in the first pass. 
%Since the context dependent features rely on the easy entity window for computation, their performance will be impacted. However, when all these features are taken together, the overall performance improves even further. This demonstrates that context is an important factor in entity disambiguation and linking.
%Our final algorithm, which utilizes all the context dependent and independent feature sets, has a precision of 63\%, recall of 87\% and f-score of 73\%. 
%
%Table \ref{LanguagePerf} shows the performance of the Lithium EDL system across various languages. We note that the test datasets for these languages are smaller. However, the algorithm's performance is comparable to that for the English dataset.

%\subsection{Comparison with baseline}
%We also compare our algorithm with a baseline algorithm that simply uses the most important context independent feature (\emph{Mention-Entity-Cooccurr}) score to disambiguate entities. Table \ref{baselinecomparison} shows the comparison of the two algorithms on the test data. The baseline algorithm has high Recall but low Precision.

\subsection{Runtime Performance}

The Lithium NLP system has been built to run in a bulk manner as well as a REST API service.
The two major challenges that we faced while developing the system were the volume of new data that we process in bulk daily and limited computational capacity. These challenges had a significant influence on our system design and algorithmic approach.

As a demonstrative example, the most consuming task in our MapReduce cluster processes around 910 million documents, with an average document size of 169 bytes, taking about 2.2ms per document. Our MapReduce cluster has around 150 Nodes each having a 2.5 GHz Xeon processor. The processing is distributed across 400 reducers. The Reduce step takes about 2.5 hrs. Each reducer task runs as a single thread with an upper bound of 7GB on memory where the processing pipeline and models utilize 3.7GB. 

A more detailed breakdown of the computational performance of our system as a function of document length is shown in Figure \ref{fig:processing_times}. The overall performance of the system is a linear function of text length. We also analyze this performance for different languages as well as for different stages of the Lithium NLP pipeline. 

%We can see that the computation is slowest for English since it has the maximum number of entities \cite{Spasojevic:dawt}.

% -- Some stats.
% CPU time spent (ms) 2,016,166,070
% Map output bytes	517,308,868,339	0	517,308,868,339
% Map output materialized bytes	153,880,824,483
% Map output records	908,428,345
% Reduce input groups	0	693,319,806	693319806
% Reduce input records	0	908428345	908428345
% Reduce output records	0	0	0
% Reduce shuffle bytes	0	153880824483	153880824483


==> papyrus paper latex/texfiles/framework.tex <==
Figure \ref{fig:papyrus} shows a high level overview of the Lithium NLP system. It has two phases:

\begin{figure*}[t]
\begin{minipage}[b]{1\linewidth} 
\centering
\includegraphics[width=\textwidth]{figures/papyruspipelinerevised.pdf}
\caption{Overview of the Lithium NLP pipeline}
\label{fig:papyrus}
\end{minipage}

\begin{minipage}[b]{1\linewidth} 
\centering
\includegraphics[width=\textwidth]{figures/papyrusstageoutput.pdf}
\caption{An example demonstrating the information extracted and added as semantic annotation at each stage of the Lithium NLP pipeline (best viewed in color)}
%\vspace{-0.1in}
\label{fig:papyrusdemo}
%\vspace{-0.1in}
\end{minipage}
\end{figure*}

\subsection{Offline Resource Generation \label{subsection:resourcegeneration}}

In this phase, we generate several dictionaries that capture language models, probabilities and relations across entities and topics, by leveraging various multi-lingual data sources. Some of these dictionaries are derived using our DAWT\footnote{\url{https://github.com/klout/opendata/tree/master/wiki_annotation}} data set \cite{Spasojevic:dawt} that consists of densely annotated wikipedia pages across multiple languages. It is 4.8 times denser than Wikipedia and is designed to be exhaustive across several domains. 

The dictionaries generated from the DAWT dataset are:

\begin{itemize}%[noitemsep, nolistsep]
  \item \textbf{Mention-Entity Co-occurrence} - This dictionary captures the prior probability that a mention $M_{i}$ refers to an entity $E_{j}$ (including \textbf{NIL} and \textbf{MISC}) within the DAWT dataset
  %our Knowledge Base (KB) (described in \cite{Spasojevic:dawt}) and corpora. 
and is equivalent to the cooccurrence probability of the mention and the entity:
 
 \small
$${{count (M_{i} \rightarrow E_{j})} \over {count (M_{i})}}$$
\normalsize

For instance, mention \emph{Michael Jordan} can link to \textbf{Michael Jordan (Professor)} or \textbf{Michael Jordan (Basketball player)} with different prior probabilities. 
Moreover, we generate a separate dictionary for each language. 

  \item \textbf{Entity-Entity Co-occurrence} - This dictionary captures co-occurrence frequencies among entities by counting all the entities that simultaneously appear within a sliding window of 50 tokens. 
Moreover, this data is accumulated across all languages and is language independent in order to capture better relations and create a smaller memory footprint when supporting additional languages. Also, for each entity, we consider only the top 30 co-occurring entities which have at least 10 or more co-occurrences across all supported languages. For instance, entity \textbf{Michael Jordan (Basketball player)} co-occurs with entities \textbf{Basketball}, \textbf{NBA} etc. while entity \textbf{Michael Jordan (Professor)} co-occurs with entities \textbf{Machine Learning}, \textbf{Artificial Intelligence}, \textbf{UC Berkeley} etc.
\end{itemize}

We also generate additional dictionaries:
\begin{itemize}%[noitemsep, nolistsep]
  \item \textbf{Entity Importance} - The entity importance score \cite{Bhattacharyya-importance} is derived as a global score identifying how important an extracted entity is for a casual observer. This score is calculated using linear regression with features capturing popularity within Wikipedia links, and importance of the entity within Freebase. We used signals such as Wiki page rank, Wiki and Freebase incoming and outgoing links, and type descriptors within our KB etc.

  \item \textbf{Topic Parents} -  This dictionary contains the parent topics for each topic in the Klout Topic Ontology \footnote{\url{https://github.com/klout/opendata/tree/master/klout_topic_ontology}} (KTO) - a manually curated ontology built to capture social media users' interests and expertise scores, in different topics, across multiple social networks. As of April 2017, it consists of roughly 8,030 topic nodes and 13,441 edges encoding hierarchical relationships among them.  

  \item \textbf{Topic Hashtags} -  This dictionary contains hashtags recommended for topics in KTO. We determine the hashtags via co-occurrence counts of topics and hashtags, importance, recency and popularity of hashtags as well popularity of topics.
  
%  \item \textbf{Entity To Topic Mapping} - %This dictionary was derived internally in order to be able to map large set of entities into the more manageable Topical ontology described above. Most of topics do map to entity directly. 
%  This dictionary essentially contains topics from the Klout Topic Ontology that are associated with the different entities in our KB. E.g. Michael Jordan, the basketball player, will be associated with the topics `Football' and `Sports'. We generate this dictionary via a weighted ensemble of several algorithms that employ entity co-occurrence and propagate the topic labels.
%  %This seed data together with link structure of wiki markup data set to derive mappings of all entities to mixture of topics.
%  A complete description of these algorithms is beyond the scope of this paper.

\end{itemize}

\subsection{Text Processing}

In the Lithium NLP system, an input text document is stored as a Protocol Buffers\footnote{\url{https://developers.google.com/protocol-buffers/}} message. The Text Processing phase of the system processes the input text document through several stages and the information (entities, topics etc.) extracted at every stage is added as a semantic annotation to the text. % in order to produce an output semantically annotated text document.% as it goes through the pipeline. 
Not all annotations are added to a document, the Lithium NLP API (explained in Section \ref{subsection:api}) allows a client application to select specific annotations. However, certain annotations such as language and tokens are prerequisites for later stages. 

The Text Processing pipeline stages are:

\begin{itemize}%[noitemsep, nolistsep]
\item \textbf{Language Detection} - This stage detects the language of the input document using an open source language detector\footnote{\url{https://github.com/shuyo/language-detection}}. This detector employs a naive Bayesian filter which uses character, spellings and script as features to classify language and estimate its probability. It has a precision of $~99\%$ for 49 languages. 
%works for %53% languages
\item \textbf{Text Normalization} - This stage normalizes the text by escaping unescaped characters and replacing special characters (e.g. diacritical marks) based on the detected language. It replaces non-ASCII punctuations and hyphens with spaces, multiple spaces with single space, converts accents to regular characters etc.

\item \textbf{Sentence Breaking} - This stage breaks the normalized text into sentences using Java Text API\footnote{\url{https://docs.oracle.com/javase/7/docs/api/java/text/BreakIterator.html}}. It can distinguish sentence breakers from other marks, such as periods within numbers and abbreviations, according to the detected language.

\item \textbf{Tokenization} - This stage converts each sentence into a sequence of tokens via the Lucene Standard Tokenizer\footnote{\url{http://lucene.apache.org/core/4_5_0/analyzers-common/org/apache/lucene/analysis/standard/StandardTokenizer.html}} for all languages and the Lucene Smart Chinese Analyzer\footnote{\url{https://lucene.apache.org/core/4_5_0/analyzers-smartcn/org/apache/lucene/analysis/cn/smart/SmartChineseAnalyzer.html}} for Chinese.
% to other languages.

\item \textbf{Entity Extraction} - This stage extracts mentions in each sentence using the Mention Entity Co-occurrence dictionary generated offline (Section \ref{subsection:resourcegeneration}).
%generated in the Offline Resource Generation phase.  %This dictionary is a rich collection of mappings between an entity and a mention. 
%Please see Section \ref{subsection:resourcegeneration} for more details about dictionary generation. 
%Note that a mention may map to multiple entities and vice versa. 
%
%Often there are multiple ways to break a sentence into a set of mentions.
A mention may contain a single token or several consecutive tokens, but a token can belong to at most one mention. 

To make this task computationally efficient, we apply a simple greedy strategy that analyzes windows of \emph{n}-grams (n $\in$ [1,6]) and extracts the longest mention found in each window. For each extracted mention, we generate multiple candidate entities. For instance, mention \emph{Android} can link to candidate entities \textbf{Android (OS)} or \textbf{Android (Robot)}.

\item \textbf{Entity Disambiguation and Linking (EDL)} - This stage disambiguates and links an entity mention to the correct candidate entity in our KB \cite{Bhargava:edl}. 
It uses several features obtained from the dictionaries generated offline (Section \ref{subsection:resourcegeneration}). These include context-independent features, such as mention-entity co-occurrence, mention-entity Jaccard similarity and entity importance, and context-dependent features such as entity entity co-occurrence and entity topic semantic similarity. It employs machine learning models, such as decision trees and logistic regression, generated using these features to correctly disambiguate a mention and link to the corresponding entity. This stage has a precision of 63\%, recall of 87\% and an F-score of 73\% when tested on an in-house dataset.

\item \textbf{Topic Projection} -  In this stage, we associate each entity in our KB to upto 10 most relevant topics in KTO. For instance, entity \textbf{Android (OS)} will be associated with the topics such as \emph{Smartphones}, \emph{Software} etc. 

We use a weighted ensemble of several semi-supervised models that employ entity co-occurrences, GloVe \cite{glove2014} word vectors, Freebase hierarchical relationships and Wikipedia in order to propagate topic labels. A complete description of this algorithm is beyond the scope of this paper.

\item \textbf{Hashtag Recommendation} - In this stage, we annotate the text with hashtags recommended based on the topics associated with the text in Topic Projection. This uses the Topic Hashtags dictionary generated offline (Section \ref{subsection:resourcegeneration})

\item \textbf{Sentiment Analysis} - In this stage, we determine the sentiment of the text (positive, negative or neutral) via lexicons and term counting with negation handling \cite{Spasojevic:actionability}. For this, we used several lexicons of positive and negative words (including SentiWordNet \cite{baccianella2010sentiwordnet, esuli2007sentiwordnet} and AFINN \cite{nielsen2011new}) as well as emoticons. We compute the sentiment score as

\small
$$
{{W_{Pos} - W_{Neg}} \over {\textrm{Log(Total \# of words in text) }+ \epsilon}}
$$
\normalsize

where $W_{Pos}$ is the weighted strength of positive words and emoticons, $W_{Neg}$ is the weighted strength of negative words and emoticons in the text and $\epsilon$ is a smoothing constant. If the score is positive and above a certain threshold, the text is classified as `Positive'. If it is below a certain threshold, the text is classified as `Negative'. If it lies within the boundary between `Positive' and `Negative' classes, the text is classified as `Neutral'. 

To handle negations, we use a \emph{lookback window}. Every time, we encounter a word from our sentiment lexicons, we look back at a window of size 3 to see if any negation words precede it and negate the weight of the sentiment word. Overall, this stage has a precision of 47\%, recall of 48\% and an F-score of 46\% when tested on an in-house dataset.

\item \textbf{Entity Metadata Decoration} - In this stage, we add the entity metadata such as its type (Person, Organization, Location, Film, Event, Book) and Location (Population, Time Zone, Latitude/Longitude).

\end{itemize}

Figure \ref{fig:papyrusdemo} demonstrates how the Lithium NLP pipeline processes a sample text ``\emph{Google CEO Eric Schmidt said that the competition between Apple and Google and iOS vs. Android is `the defining fight of the tech industry'.}" and adds the annotations at every stage.

\subsection{REST API}\label{subsection:api}

The Lithium NLP system provides a REST API via which client applications can send a text document as request and receive the annotated text as JSON response. A snippet of an annotated response (which is in our text proto format\footnote{\url{https://github.com/klout/opendata/blob/master/wiki_annotation/Text.proto}}) received through the API is shown in Listing \ref{jsonresponse}. Note that the disambiguated entities are also linked to their Freebase ids and Wikipedia links. \\ \\ 

\begin{lstlisting}[language=json,basicstyle=\scriptsize,firstnumber=1,breaklines=true,caption=JSON of annotated text summary,label=jsonresponse]
{
  "text": "Vlade Divac Serbian NBA player used to play for LA Lakers.",
  "language": "en",
  "annotation_summary": [{
      "type": "ENTITY",
      "annotation_identifier": [{
          "id_str": "01vpr3",
          "id_url": "https://en.wikipedia.org/wiki/Vlade_Divac",
          "score": 0.9456,
          "type": "PERSON"
        }, {
          "id_str": "05jvx",
          "id_url": "https://en.wikipedia.org/wiki/NBA",
          "score": 0.8496,
          "type": "ORGANIZATION"
        }, ...
      }]
  },
  {
    "type": "KLOUT_TOPIC",
    "annotation_identifier": [{
      "id_str": "6467710261455026125",
      "id_readable": "nba",
      "score": 0.7582
    }, {
      "id_str": "8311852403596174326",
      "id_readable": "los-angeles-lakers",
      "score": 0.66974
    }, {
      "id_str": "8582816108322807207",
      "id_readable": "basketball",
      "score": 0.5445
    }, ...]
  },
  {
    "type": "HASHTAG",
    "annotation_identifier": [{
      "id_str": "NBA",
      "score": 54285.7515
    }, {
      "id_str": "NBAPlayoffs",
      "score": 28685.6006
    }, ...]
  }],
   "sentiment": 0.0
}
\end{lstlisting}

\subsection{Performance}\label{subsection:performance}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.47\textwidth,height=70mm]{figure/papyrus_performance_per_language_per_stage/eps/en_performance_all_stages.pdf}
  \caption{Lithium NLP performance per processing stage (best viewed in color)}
  \label{fig:stage_performance}
   \vspace{-0.1in}
\end{figure}

Figure \ref{fig:stage_performance} shows the computational performance per processing stage of the Lithium NLP system.
The overall processing speed is about 22ms per 1kb of text. As shown, the time taken by the system is a linear function
of text size. The EDL stage takes about $80\%$ of the processing time.

==> papyrus paper latex/texfiles/introduction.tex <==

\begin{figure*}[t]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/ExpertiseScore.png}
    \caption{A user's inferred expertise topics}
    %        \vspace{-0.1in}
    \label{fig:expertise_score}
  \end{minipage}
  \qquad
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/ContentDiscovery.png}
    \caption{Content Personalization}
     %           \vspace{-0.1in}
    \label{fig:content_discovery}
  \end{minipage}
 % \vspace{-0.1in}
\end{figure*}

Social media has become one of the major means for communication and content production. As a result, industrial systems that possess the capability to process rich user generated content from social media platform have several real-world applications. Furthermore, due to the content style, size and heterogeneity of information (e.g. text, emoticons, hashtags etc.) available on social media, novel NLP techniques and systems that are designed specifically for such content and can potentially integrate or learn information from different sources are highly useful and applicable. 

However, NLP on social media data can be significantly complex and challenging due to several reasons:
\begin{itemize}%[noitemsep, nolistsep]
%\item Ambiguity - The same entity mention can refer to different real world entities in different contexts. A clear example of ambiguity is the mention \emph{Michael Jordan} which can refer to the basketball player in certain context or the machine learning professor from Berkeley. To the discerning human eye, it may be easy to identify the correct entity, but any EDL system attempting to do so needs to rely on contextual information when faced with ambiguity.
\item \textbf{Noisy unnormalized data} - Social media data is much more informal than traditional text and less consistent in language in terms of style, tone etc. It involves heavy usage of slang, jargons, emoticons, or abbreviations which usually do not follow formal grammatical rules. Hence, novel NLP techniques need to be developed for such content.
\item \textbf{Multi-lingual content} - Social media data poses an additional challenge to NLP practitioners because the user generated content on them is often multi-lingual. Hence, any NLP system processing real world data from the web should be able to support multiple languages in order to be practical and applicable. %Unfortunately, this is a challenge that has not been given enough attention. 
\item \textbf{Large scale datasets} - State-of-the-art NLP systems should be able to work on large scale datasets such as social media data, often involving millions of documents. Moreover, these systems need to have low resource consumption in order to scale to such datasets in a finite amount of time. In addition, in order to be applicable and practical, they should be able to run on off-the-shelf commodity machines. 
\item \textbf{Rich set of information} - In order to be cost-efficient, state-of-the-art NLP systems need to be exhaustive in terms of information extracted\footnote{\url{https://en.wikipedia.org/wiki/Information_extraction}} from social media text. This includes extracting entities of different types (such as professional titles, sports, activities etc.) in addition to just named entities (such as persons, organizations, locations etc.), inferring fine-grained and coarse-grained subject matter topics (sports, politics, healthcare, basketball), text sentiment, hashtags, emoticons etc. %Social media data often provides 
%However, as we show later, most existing systems focus on extracting named entities only.
\end{itemize}

In this paper, we present the Lithium NLP\footnote{A screencast video demonstrating the system is available at \url{https://youtu.be/U-o6Efh6TZc}} system which addresses these challenges. It is a resource-constrained, high-throughput and language-agnostic system for information extraction from noisy user generated text such as that available on social media. It is capable of extracting a rich set of information including entities, topics, hashtags and sentiment. Lithium NLP currently supports multiple languages including Arabic, English, French, German, Italian and Spanish. It supports large scale data from several social media platforms such as Twitter, Facebook, Linkedin, etc. by processing about $500M$ new social media messages, and $0.5M$ socially relevant URLs shared daily. Since it employs statistical NLP techniques, it uses the large scale of the data to help overcome the noisiness.

Lithium NLP is currently incorporated in several Lithium products. It enables consumer products like Klout\footnote{\url{https://klout.com}} - a platform which integrates users' data from multiple social networks such as Twitter, Facebook, Instagram, Linkedin, GooglePlus, Youtube, and Foursquare, in order to measure their online social influence via the \emph{Klout Score\footnote{\url{https://klout.com/corp/score}}} \cite{rao2015kloutScore}. On Klout, it is used to model users' topics of interest \cite{nemanja-lasta} and expertise \cite{Spasojevic2016:experts} by building their topical profiles. Figure \ref{fig:expertise_score} shows an example of a user's topics of expertise, as inferred on Klout. Currently, we build topical profiles for more than $600M$ users. These profiles are further used to recommend personalized content to these users by matching their topics of interest or expertise with content topics as this leads to better user engagement. 
An example of content personalization is shown in Figure \ref{fig:content_discovery}. The user scores and topics are also available via the GNIP PowerTrack API\footnote{\url{http://support.gnip.com/enrichments/klout.html}}.
%On Klout, the Lithium NLP system by its $600M$ daily active users. 

Lithium NLP also enables enterprise products such as Lithium's social media management tools\footnote{\url{https://www.lithium.com/products/social-media-management/}} - Lithium Reach and Lithium Response. It is used to analyze $20+M$ new daily engagements across Lithium's 400+ communities\footnote{\url{https://www.lithium.com/products/online-communities/}}. In the past, a version of Lithium NLP had been used to enable user targeting applications such as Klout Perks\footnote{\url{https://goo.gl/vtZDqE\#Klout_Perks}} (influencer reward platform), Cinch\footnote{\url{https://goo.gl/CLcx9p\#Cinch}} (Q\&A app), and Who-To-Follow recommendations. These involved selecting a group of users for targeting based on given topics and other filtering criteria.

%As mentioned earlier, the Lithium NLP system is currently incorporated in several Lithium products including Klout, Lithium Reach and Response. Its applications include:

%\begin{itemize}[nolistsep,noitemsep]
%\item \textbf {User modeling} - Building topical profiles of users on Klout to model their interests and expertise.  
%We derive \textbf{topic profiles} of individual users by analyzing their social media texts and URLs with the pipeline. A profile contains two types of topics 

%\begin{itemize}[noitemsep, nolistsep]
%  \item Topics that are interesting to the user \cite{nemanja-lasta} 
%  \item Topics on which the user is an expert \cite{Spasojevic2016:experts}
%\end{itemize}

%\item \textbf{User Targeting} - 
%\end{itemize}



==> papyrus paper latex/texfiles/knowledgebase.tex <==
Our Knowledge Base (KB) consists of about 1 million Freebase machine ids for entities 
%Entity ids in our knowledge base (KB) were chosen from a subset of Freebase entities that map to Wikipedia entities.
that were chosen from a subset of  all Freebase entities that map to Wikipedia entities.
We  prefer to use Freebase rather than Wikipedia as our KB since in Freebase, the same id represents a unique entity across multiple languages.
%Within research community, Wikidata Knowledge emerged as the new standard.Similar to Freebase - Wikidata KB same ids map across across multiple languages,and maps in almost 1:1 correspondence to Freebase id space (for entities that have Wikipedia page).
Due to limited resources and usefulness of the entities, our KB contains approximately 1 million most important entities from among all the Freebase entities. 
This gives us a good balance between coverage and relevance of entities for processing common social media text.
%The total size of English Wikipedia articles is close to 5M, with more than 40M articles across all 288 languages.
Section \ref{subsection:resourcegeneration} explains how entity importance is calculated, which enables us to rank the top 1 million Freebase entities.

In addition to the KB entities, we also employ two special entities: \textbf{NIL} and \textbf{MISC}.
%Both are utilized in order to try to capture the true probability of entity given an mention.
\textbf{NIL} entity indicates that there is no entity associated with the mention, eg. mention `the' within the sentence may link to entity \textbf{NIL}. This entity is useful especially when it comes to dealing with stop words and false positives. \textbf{MISC} indicates that the mention links to an entity which is outside the selected entity set in our KB. 
%For example, in Wikipedia phrase `1982' may link to `1982 NCAA Mens Basketball tournament', or `Yugoslavian soccer team of 1982 FIFA Championship', none of which is in our set and hence will map to \textbf{MISC}.

==> papyrus paper latex/texfiles/relatedwork.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.47\textwidth]{figure/papyrus_vs_aida_overall/eps/papyrus_vs_aida_overall.eps}
  \caption{AIDA vs. Lithium NLP  Comparison on \textbf{a)} Text processing runtime \textbf{b)} Extracted entity count  (best viewed in color)}
  \label{fig:aida_vs_lithium}
 %  \vspace{-0.1in}
\end{figure}


\begin{table*}[t]
\begin{minipage}[b]{1\linewidth} 
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
 & \textbf{Lithium NLP} & \textbf{Google NL} & \textbf{Open Calais} & \textbf{Alchemy API} & \textbf{Stanford CoreNLP} & \textbf{Ambiverse} & \textbf{Twitter NLP}\\
  \hline
  \textbf{Named Entities} & X & X & X & X & X & X & X \\
    \hline
  \textbf{Other Entities} & X & X & X & X & X & &\\
\hline
  \textbf{Topics (fine-grained)} & X &  &  &  &  &  &\\
  \hline
  \textbf{Topics (coarse-grained)} & X	&  & X & X &  & &  \\
\hline
  \textbf{Hashtags} & X &  &  &  &  &  &\\
\hline
  \textbf{Document Sentiment} & X &  &  & X & X & &\\
\hline   
  \textbf{Entity level Sentiment} &  & X &  & X & & &\\
  \hline
  \textbf{Entity types} & X & X & X & X &X &X & X\\
  \hline
    \textbf{Relationships} &  &  & X & X &X & &\\
  \hline
      \textbf{Events} &  &  &  &  & & & X\\
  \hline
%    \textbf{Syntax (POS/Parsing etc.)} &  & X &  & X &X &  \\
  %\hline
\end{tabular}}
%\vspace{-0.1in}
\caption{Comparison of information extracted by Lithium NLP with existing NLP systems}
\label{table:CapabilitiesComparison}
\end{minipage}

\begin{minipage}[b]{1\linewidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
 & \textbf{Lithium NLP} & \textbf{Google NL} & \textbf{Open Calais}  & \textbf{Alchemy API}  & \textbf{Stanford CoreNLP} & \textbf{Ambiverse} & \textbf{Twitter NLP}\\
\hline
 \textbf{Supported}  & Arabic, English, & Chinese, English, French, & English,  & English, French, German,  & Arabic, Chinese,  & English, German, & English\\ 
 \textbf{Languages} &  French, German,  &  German, Italian, Japanese,  & French, &  Italian, Portuguese, Russian,  & English, French,  & Spanish,  & \\ 
  &  Italian, Spanish & Korean, Portugese, Spanish & Spanish &  Spanish, Swedish  & German, Spanish & Chinese & \\ 
  \hline
\end{tabular}}
%\vspace{-0.1in}
\caption{Comparison of languages supported by Lithium NLP with existing NLP systems}
\label{table:LanguagesComparison}
%\vspace{-0.1in}
\end{minipage} 
\end{table*}

Currently, due to limited resources at our end and also due to inherent differences in the Knowledge Base (Freebase vs Wikipedia and others), test dataset, and types of information extracted (entities, topics, hashtags etc.), a direct comparison of the Lithium NLP system's performance (in terms of precision, recall and f-score) with existing academic and commercial systems such as Google Cloud NL API\footnote{\url{https://cloud.google.com/natural-language/}}, Open Calais\footnote{\url{http://www.opencalais.com/opencalais-demo/}}, Alchemy API\footnote{\url{https://alchemy-language-demo.mybluemix.net/}}, Stanford CoreNLP\footnote{\url{http://corenlp.run/}} \cite{manning2014stanford}, Ambiverse/AIDA\footnote{\url{https://www.ambiverse.com/}} \cite{nguyen2014aida} and Twitter NLP\footnote{\url{https://github.com/aritter/twitter_nlp}} \cite{ritter2011named,Ritter12} is not possible. Hence, we compare our system with some of them on a different set of metrics.

\subsection{Comparison on runtime and entity density}

We compare the runtime of Lithium NLP and AIDA across various text sizes.
As shown in Figure \ref{fig:aida_vs_lithium}, Lithium NLP is on an average 40,000 times faster than AIDA whose slow runtime can be attributed mainly to Stanford NER. In addition to speed, we also compare the number of entities extracted per kb of text. As shown, Lithium NLP extracts about $2.8$ times more entities than AIDA.

\subsection{Comparison on information extracted}

Table \ref{table:CapabilitiesComparison} compares the types of information extracted by Lithium NLP system with existing systems. In this comparison, we explicitly differentiate between named entities (Person, Location etc.) and other entity types (Sports, Activities) as well as fine-grained topics (Basketball) and coarse-grained topics (Sports) to demonstrate the rich set of information extracted by Lithium NLP. As evident, most other systems do not provide the rich set of semantic annotations that Lithium NLP provides. A majority of the systems focus on recognizing named entities and types with only a few focusing on sentiment and coarse-grained topics as well. In contrast, Lithium NLP extracts, disambiguates and links named and other entities, extracts subject matter topics, recommends hashtags and  also infers the sentiment of the text.

\subsection{Comparison on languages}

Table \ref{table:LanguagesComparison} compares the languages supported by the Lithium NLP system with existing systems. As evident, Lithium supports 6 different languages which is at par and in some cases, more than existing systems.







==> papyrus paper latex/texfiles/tuning.tex <==

%\begin{figure}
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=75mm ,height=60mm]{figures/FirstPassthresholdsPR.pdf}
%    \caption{Precision Recall curve for different values of first pass parameters $\lambda_{1}$ and $\lambda_{2}$}
%    \label{fig:firstpasspr}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=75mm ,height=60mm]{figures/WindowsizePR.pdf}
%    \caption{Precision Recall curve for different values of window size}
%    \label{fig:windowsizepr}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=75mm ,height=60mm]{figures/NoneMarginGainPR.pdf}
%    \caption{Precision Recall curve for different values of NONE margin gain}
%    \label{fig:nonemargingainpr}
%  \end{subfigure}
%  \label{Parameter Tuning Results}
%  \caption{Precision Recall curves for parameter tuning}
%\end{figure}


%We use part of our training data (generated as explained in Section \ref{data_set}) for tuning the hyper parameters. We split the data in a 7:3 ratio and use 70\% of the data for training. We use 20\% for testing and 10\% for validation.
Our algorithm uses four different hyperparameters - 2 in the first pass and 2 in the second pass. These are:

\begin{itemize}[noitemsep,nolistsep]
\item Easy mention disambiguation threshold with \textbf{NIL} ($\lambda_{1}$) - This threshold is used to disambiguate easy mentions which have 2 candidate entities and one of them is the \textbf{NIL} entity.
\item Easy mention disambiguation threshold ($\lambda_{2}$) - This threshold is used to disambiguate easy mentions which have 3 or more candidate entities but the mention maps to one of them with a very high prior probability.
%\end{itemize}

%The second pass parameters are:
%\begin{itemize}[noitemsep,nolistsep]
\item \textbf{NIL} margin of gain threshold ($\lambda_{3}$) - This threshold is used in the second pass to disambiguate entities when multiple or none of the candidates are labeled `True'.
\item Window size (\emph{W}) - This parameter represents the size of the easy entity window around each hard entity.
\end{itemize}

Using the process described in Section \ref{data_set}, we generated a ground truth validation set of 10 English Wikipedia pages which had a total of 7242 mentions and 23,961 candidate entities. We used parameter sweeping experiments to determine the optimal value of these parameters. We measured the performance (in terms of precision, recall and f-score) of the algorithm on the validation set with different parameter settings and picked the parameter values that had the best performance. 
%Figure \ref{fig:firstpasspr} shows the Precision-Recall curve for $\lambda_{1}$ $\in$ [0.85,0.95] and $\lambda_{2}$ $\in$ [0.75,0.95]. Figure \ref{fig:windowsizepr} shows the Precision-Recall curve for \emph{w} $\in$ [25,400]. Figure \ref{fig:nonemargingainpr} shows the Precision-Recall curve for $\lambda_{3}$ $\in$ [0.3,0.55].  
Based on our experiments, we set the optimal value of $\lambda_{1}$ as 0.75, $\lambda_{2}$ as 0.9, \emph{W} as 400 and $\lambda_{3}$ as 0.5. %as they achieve the highest Precision, Recall and F-score on the validation set.




==> texfiles/algorithm.tex <==
%\begin{algorithm*}[t]
%    \SetAlgoLined
%\KwInput{Text $T_{i}$ with extracted mentions $\mathbb{M}_{all}$ and a set of candidate entities for each mention}
%\KwOutput{Text $T_{i}$ with extracted mentions $\mathbb{M}_{all}$ and a unique disambiguated entity for each mention}
%\tcp{First pass - Disambiguate the easy mentions}
%$\mathbb{M}_{easy}$ $\leftarrow$ Easy mentions obtained from the first pass on $T_{i}$\;
%    $\mathbb{E}_{easy}$ $\leftarrow$ Disambiguated easy entities obtained from the first pass on $T_{i}$\;
%    Document Context $C(T_{i})$  $\leftarrow$ $C(T_{i})$ + $\mathbb{E}_{easy}$ \; 
%    $\mathbb{M}_{hard}$ $\leftarrow$ $\mathbb{M}_{all}$ - $\mathbb{M}_{easy}$\;
%    \tcp{Second pass - Iterate over the hard mentions}
%    \ForEach{Mention \emph{$M_{j}$} $\in$ $\mathbb{M}_{hard}$} {
%    $\mathbb{H}_{j}$ $\leftarrow$ Candidate entities of $M_{j}$\;
%    \tcp{Iterate over the candidate entities of a hard mention}
%    \ForEach{Entity \emph{$E_{k}$} $\in$ $\mathbb{H}_{j}$} {
%    Entity Context  C'($E_{k}$) $\leftarrow$ C'($E_{k}$) + $\mathbb{E}'_{k}$ (set of easy entities in a window around $E_{k}$) \;
%	$F_{E_{k}}$ $\leftarrow$ Generate feature vector of context independent and dependent features values for $E_{k}$ using C'($E_{k}$)\;
%	Classify $F_{E_{k}}$ as one of \emph{$\left\{\text{True, False}\right\}$} using Decision Tree classifier\;
%	$S_{E_{k}}$ $\leftarrow$ Final score for $E_{k}$ generated using Logistic Regression model weights\;
%	Add $S_{E_{k}}$ to set $S_{j}$ (Set of candidate entity scores for \emph{$M_{j}$})\;
%    }
%    \tcp{Final disambiguation - select one of the candidate entities as disambiguated entity $D_{j}$ for \emph{$M_{j}$}}
%    	\uIf{Only one $E_{k}$ $\in$ $\mathbb{H}_{j}$ labeled as  \emph{True}} {
%	 	$D_{j}$ $\leftarrow$ $E_{k}$ labeled as \emph{True}\;
%	}  \uElse {
%	\uIf{Multiple $E_{k}$ labeled as True}{
%		$D_{j}$ $\leftarrow$ Highest scoring $E_{k}$ labeled as \emph{True}\;
%	}  \uElseIf{None of $E_{k}$ labeled as True}{
%		$D_{j}$ $\leftarrow$ $\argmax$ ($S_{E_{k}}$)\;
%	}
%	\uIf{$D_{j}$ is \textbf{NIL} and \emph{NIL\_MARGIN\_GAIN} < threshold} {
%		$D_{j}$ $\leftarrow$ $\argmax$ ($S_{j}$ - $S_{D_{j}}$)\;
%	}
%}
%}
%    \Return{Text with extracted mentions and disambiguated entities\;}
%      \caption{Lithium EDL algorithm}
%    \label{alg:nedl}
%\end{algorithm*}

%As mentioned earlier, the Lithium EDL system uses a two pass algorithm for disambiguating and linking entities. 

Algorithm \ref{alg:nedl} describes the Lithium EDL two-pass algorithm. %In the first pass, we disambiguate easy entities while in the second pass, we utilize the easy entities within a given window to disambiguate hard entities. 
We discuss it in detail now (the design choices for various parameters are explained in Section \ref{section:tuning}).

\subsection{First pass \label{firstpass}}
The first pass of the algorithm iterates over all mentions in the document text and disambiguates mentions that have:
\begin{itemize}[noitemsep,nolistsep]
\item Only one candidate entity: In this case, the algorithm disambiguates the mention to the lone candidate entity.
\item Two candidate entities with one being \textbf{NIL}/\textbf{MISC}:  In this case, the algorithm disambiguates the mention to the candidate entity with high \emph{Mention-Entity-Cooccurr} prior probability (above $\lambda_{1}$ - Easy Mention Disambiguation threshold with \textbf{NIL}).
%Based on our experiments on a validation set (which consists of 10 Wikipedia pages generated using the process described in Section \ref{data_set}), we set this confidence threshold as 0.75.
\item Three or more candidate entities with one entity mapping with very high prior: In this case, the algorithm disambiguates the mention to the candidate entity with high \emph{Mention-Entity-Cooccurr} prior probability (above $\lambda_{2}$ - Easy Mention Disambiguation threshold). 
%Based on experiments on the validation set, we set the confidence threshold as 0.9. 

\end{itemize}

Mentions disambiguated in the first pass constitute the set $\mathbb{M}_{easy}$ and their corresponding disambiguated entities constitute the set $\mathbb{E}_{easy}$. The remaining ambiguous mentions constitute the set $\mathbb{M}_{hard}$ and are disambiguated in the second pass.

\subsection{Second pass}
The second pass of the algorithm uses several context-independent and context-dependent features as well as supervised classifiers to label and score the candidate entities for each hard mention and finally disambiguate it. 

\subsubsection{\textbf{Features}} \label{sec:features}

We use several language agnostic features to classify each candidate entity for each hard mention as `True' or `False'. These include both context-independent (useful for disambiguating and linking entities in short and sparse texts such as tweets) as well as context-dependent features (useful for disambiguating and linking entities in long and rich text). Each feature produces a real value in [0.0,1.0].

The context independent features are:

\begin{itemize}[noitemsep,nolistsep]

\item \textbf{Mention-Entity Cooccurrence} (\emph{Mention-Entity-Cooccurr}) - This feature value is equal to the \emph{Mention-Entity-Cooccurr} prior probability.

\item \textbf{Mention-Entity Jaccard Similarity} (\emph{Mention-Entity-Jaccard}) - This reflects the similarity between the mention $M_{i}$ and the representative name of a candidate entity $E_{j}$. The mention and the entity display names are first tokenized and the Jaccard similarity is then computed between the token sets as
%Can we describe why this feature is useful or what are the additional information this feature tries to capture?
\small
$$
%\emph{Mention-Entity-Jaccard} = {{Tokens(M_{i}) \cap Tokens(E_{j})} \over {Tokens(M_{i}) \cup Tokens(E_{j})}}
{{Tokens(M_{i}) \cap Tokens(E_{j})} \over {Tokens(M_{i}) \cup Tokens(E_{j})}}
$$
%This feature produces a real value in [0.0,1.0].
\normalsize
For instance, the mention \emph{Marvel} could refer to the entities \emph{Marvel Comics} or \emph{Marvel Entertainment}, both of which have a Jaccard Similarity of 0.5 with the mention.

\item \textbf{Entity Importance} (\emph{Entity-Importance}) - This reflects the importance or the relevance of the candidate entity as determined by an entity scoring and ranking algorithm \cite{Bhattacharyya-importance} which ranks the top 1 million entities occurring in our KB. For instance, the entity \emph{Apple Inc.} has an importance of 0.66 while \emph{Apple (fruit)} has an importance of 0.64 as ranked by the Entity Scoring algorithm.

\end{itemize}

\begin{figure}[t]
\centering
\includegraphics[width=75mm ,height=35mm]{figures/TopicOntologySemanticDistance.pdf}
\vspace{-0.1in}
\caption{Semantic distance between topics in Klout Topic Ontology Space}
\label{fig:topicsimdist}
\vspace{-0.1in}
\end{figure}

For the following context dependent features, we assume that for a candidate entity $E_{i}$, we maintain an entity context C'($E_{i}$) which contains a window $\mathbb{E}'_{i}$ of \emph{W} disambiguated easy entities immediately surrounding $E_{i}$.

\begin{itemize}[noitemsep,nolistsep]
\item \textbf{Entity Entity Cooccurrence} (\emph{Entity-Entity-Cooccurr}) - 
%The entity context for each hard mention in the text
%, as computed after the First Pass of our algorithm (Section \ref{firstpass}), includes the easy mentions that have been disambiguated in the immediate window of the hard mention. 
This feature value is equal to the averaged co-occurrence of a candidate entity with the disambiguated easy entities in $\mathbb{E}'_{i}$ and is computed as:
%For instance, for a candidate entity $E_{i}$ and the set $\mathbb{E}'_{i}$ of easy entities in $E_{i}$'s window, the feature is computed as:
\small
%\emph{Entity-Entity-Cooccurr}  = 
$$
{\sum_{j=1}^{W} Co-occurrence-count (E_{i}, E_{j}) \over {W}} \forall E_{j} \in  \mathbb{E}'_{i}
$$
%This feature produces a real value in [0.0,1.0].
\normalsize

\item \textbf{Entity Entity Topic Semantic Similarity} (\emph{Entity-Entity-Topic-Sim}) - As mentioned in Section \ref{subsection:OfflineDictionary}, each entity in our KB is associated with a finite number of topics in our topic ontology. For instance, entity \emph{Apple Inc.} maps to the topic `Apple' and \emph{Google Inc.} maps to the topic `Google' while `\emph{Apple (fruit)}' will map to the topic `Food'. Figure \ref{fig:topicsimdist} shows a partial view of the ontology for the above mentioned topics.  
%A complete description of the Topic Ontology is beyond the scope of this paper.

For each candidate entity $E_{i}$ of a hard mention $M_{i}$, we compute the minimum \emph{semantic distance} of its topics with topics of each entity in $\mathbb{E}'_{i}$ over all possible paths in our topic ontology space. The similarity is the inverse of the distance. For instance, consider the hard mention \emph{Apple}, having two candidate entities - \emph{Apple Inc.} and \emph{Apple (fruit)} for it, and $\mathbb{E}'_{i}$ containing the entity \emph{Google Inc.} which has been disambiguated. As shown in Figure \ref{fig:topicsimdist}, the semantic distance between the topics for \emph{Apple Inc.} and \emph{Google Inc.} is 4 while the semantic distance between the topics for \emph{Apple (fruit)} and \emph{Google Inc.} is 5. As a result, it is more likely that \emph{Apple} disambiguates to \emph{Apple Inc}. 

Thus, we first determine the set of topics $\mathbb{T}_{i}$ that the candidate entity $E_{i}$ is associated with. For each entity $E_{j}$ in $\mathbb{E}'_{i}$, we generate the set of topics $\mathbb{T}_{j}$. The feature value is computed as
\small
$$
\max {1 \over distance (t_{i}, t_{j})} \forall t_{i} \in \mathbb{T}_{i}, t_{j} \in \mathbb{T}_{j}
$$
\normalsize
\end{itemize}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth,height=80mm]{figures/RunningExample.pdf}
\vspace{-0.3in}
\caption{Disambiguation of a sample sentence (best viewed in color)}
\label{fig:sample}
 \vspace{-0.1in}
\end{figure*}

\subsubsection{\textbf{Classification and Scoring}}

As a penultimate step in the second pass, the computed features are combined into a feature vector for a candidate entity and the Decision Tree classifier labels the feature vector as `True' or `False'. In addition, for each candidate entity, we also generate final scores using weights generated by the Logistic Regression classifier that we trained in Section \ref{subsubsec:class}. We use an ensemble of the two classifiers in the final disambiguation step as it helps overcome the individual bias of each classifier.
%Needs to explain why we are not using the score from Decision Tree.

\subsubsection{\textbf{Final Disambiguation}}
The final disambiguation step needs to select one of the labeled candidate entities as the disambiguated entity for the mention. However, multiple cases arise at the time of disambiguation:
\begin{itemize}[noitemsep,nolistsep]
\item Only one candidate entity is labeled as `True'- Here, the algorithm selects that entity as the disambiguated entity for the given mention.
\item Multiple candidate entities labeled  as `True'  - Here, the algorithm selects the highest scoring entity (from among those labeled `True') as the disambiguated entity except when this entity is \textbf{NIL}/\textbf{MISC}. In that case, the algorithm checks the \emph{margin of gain} or the score difference between the \textbf{NIL}/\textbf{MISC} entity and the next highest scoring entity that is labeled `True'. If the margin of gain is less than a threshold (less than \textbf{NIL} margin of gain threshold, $\lambda_{3}$) then the next highest scoring entity (from among those labeled `True') is selected.
\item All candidate entities labeled as `False' - Here, the algorithm selects the highest scoring entity as the disambiguated entity except when this entity is \textbf{NIL}/\textbf{MISC}. In that case, the algorithm checks the margin of gain for this entity over the next highest scoring entity. If the margin of gain is less than a threshold (less than \textbf{NIL} margin of gain threshold, $\lambda_{3}$) then the next highest scoring entity is selected.
\end{itemize}
%Based on our experiments on the validation set, we set the \emph{margin of gain} as 0.5

\subsection{Demonstrative Example}\label{sec:demoex}

To demonstrate the efficacy of our algorithm, let's disambiguate the sample text: 
\emph{``Google CEO Eric Schmidt said that the competition between Apple and Google and iOS vs.  Android is `the defining fight of the tech industry.' ".} 

Figure \ref{fig:sample} walks through the disambiguation of the sample text. The Text Preprocessing stages extract the mentions (highlighted in bold) and generate the candidate entities and the prior cooccurrence scores for each mention\footnote{Though our algorithm utilizes the Freebase machine id for each candidate entity, we only show the entity name for clarity.}. 
As shown, the extracted mentions and their candidate entities are:
\begin{itemize}[noitemsep,nolistsep]
\item \emph{Google} - \textbf{NIL} and \emph{Google Inc.}
\item \emph{CEO} - \textbf{NIL} and \emph{Chief Executive}
\item \emph{Eric Schmidt} - \textbf{NIL} and \emph{Eric Schmidt}
\item \emph{Apple} - \textbf{NIL}, \emph{Apple (fruit)}, \emph{Apple Inc.} and \emph{Apple Records}
\item \emph{iOS} - \textbf{NIL} and \emph{iOS}
\item \emph{Android} - \textbf{NIL}, \emph{Android (OS)} and \emph{Android(robot)}
\item \emph{tech industry} - \emph{Technology}
\end{itemize}
In the first pass, the algorithm disambiguates the easy mentions. Based on their high prior scores and number of candidate entities, it disambiguates \emph{Eric Schmidt}, \emph{iOS} and \emph{tech industry} (highlighted in color) to their correct entities. 
In the second pass, it uses the easy mention window and computes several context dependent and independent features to score and classify the candidate entities of the hard mentions. Note that for the purpose of clarity and simplicity, we are not walking through the feature and final score computation. As shown, for the remaining hard entities, it has classified the candidate entities as `True' or `False'.
In the final disambiguation step, it selects one of the labeled entities as the correct disambiguated entity. In the sample sentence, for all the mentions, only one of the candidate entities is labeled as `True', and hence the algorithm selects that entity  as the disambiguated entity for each mention.

%Its quite evident that our EDL system can recognize several entities mentioned in the text and utilize this rich annotated content to understand the topics or the categories the text is about as well as 



==> texfiles/applications.tex <==
\begin{figure*}[t]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/ExpertiseScore.png}
    \caption{Topics of expertise a User }
            \vspace{-0.1in}
    \label{fig:expertise_score}
  \end{minipage}
  \qquad
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/ContentDiscovery.png}
    \caption{Content Personalization}
                \vspace{-0.1in}
    \label{fig:content_discovery}
  \end{minipage}
 % \vspace{-0.1in}
\end{figure*}

As mentioned earlier, the Lithium NLP system is currently incorporated in several Lithium products including Klout, Lithium Reach and Response. Its applications include:

\begin{itemize}[nolistsep,noitemsep]
\item \textbf {User modeling} - Building topical profiles of users on Klout to model their interests and expertise.  An example of user expertise topics is shown in Figure \ref{fig:expertise_score}. Currently, we build topical profiles for more than 600M users which are also available via GNIP PowerTrack\footnote{\url{http://support.gnip.com/enrichments/klout.html}}.
%We derive \textbf{topic profiles} of individual users by analyzing their social media texts and URLs with the pipeline. A profile contains two types of topics 

%\begin{itemize}[noitemsep, nolistsep]
%  \item Topics that are interesting to the user \cite{nemanja-lasta} 
%  \item Topics on which the user is an expert \cite{Spasojevic2016:experts}
%\end{itemize}
\item \textbf {Content Personalization} - We apply these topic profiles to recommend content to users by matching user and content topics as this leads to better user engagements. An example of content personalization on a Lithium product is shown in Figure \ref{fig:content_discovery}. %This tool is integrated into \url{https://klout.com} and \url{https://www.lithium.com/products/social-media-management/} 

\item \textbf{User Targeting} - This involves selecting a group of users for targeting based on given topics and other filtering criteria. Over the course of time, a version of Lithium NLP had been used to enable targeting applications such as Klout Perks\footnote{\url{https://goo.gl/vtZDqE\#Klout_Perks}} (influencer reward platform), Cinch\footnote{\url{https://goo.gl/CLcx9p\#Cinch}} (Q\&A app), and Who-To-Follow recommendations.

\end{itemize}


==> texfiles/dataset.tex <==
Since our goal is to build a language-agnostic NLP system, we needed a dataset that scales across several languages and also has good annotation density and coverage. Unfortunately, such a dataset is not readily available. 
Hence, we generated a ground truth data set for our NLP system, the Densely Annotated Wikipedia Text (DAWT) \cite{Spasojevic:dawt}, 
%used for derivation of the offline dictionaries and training data was based on
using densely Wikified \cite{Mihalcea:2007:WLD:1321440.1321475} or annotated Wikipedia articles. 
Wikification is entity linking with Wikipedia as the KB. We started with Wikipedia data dumps\footnote{\url{https://dumps.wikimedia.org/}},
which were further enriched by introducing more hyperlinks in the existing document structure. 
Our main goals when building this data set were to maintain high precision and increase linking coverage. 
As a last step, the hyperlinks to Wikipedia articles in a specific language were replaced with links to their Freebase ids to adapt to our KB. The densely annotated Wikipedia articles had on an average 4.8 times more links than the original articles.

==> texfiles/evaluation.tex <==
%\begin{table}[t]
%\centering
%\begin{tabular}{|c|c|c|}
%\hline
% & \multicolumn{2}{|c|}{\textbf{Ground Truth Label}}  \\
% \cline{2-3}
%\textbf{Predicted Label}  & Correct Entity & \textbf{NIL} \\
%\hline
%  Correct Entity &TP & FP\\
%\hline
% Wrong Entity& FP & FP\\
%\hline
% \textbf{NIL} & FN & TN\\
%\hline
%\end{tabular}
%%\vspace{-0.1in}
%\caption{Confusion matrix for our EDL system}
%\label{PositivesNegatives}
%\vspace{-0.3in}
%\end{table}

%\begin{table*}[!th]
%\centering
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\textbf{Features} & \textbf{Precision} & \textbf{Recall} & \textbf{Accuracy} & \textbf{F-score}\\
%\hline
% \emph{Mention-Entity-Cooccurr} (context independent) & 0.65 & 0.75 & 0.70 & 0.62\\
%\hline
%\emph{Mention-Entity-Jaccard} (context independent) & 0.47 & 0.93 & 0.48 & 0.63\\
% \hline
%\emph{Entity-Importance} (context independent) & 0.50 & 0.90 & 0.50 & 0.65\\
% \hline
%\emph{Entity-Entity-Cooccurr} (context dependent) & 0.54 & 0.91 & 0.54 & 0.68\\
% \hline
%\emph{Entity-Entity-Topic-Sim} (context dependent) & 0.49 & 0.88 & 0.49 & 0.63\\
% \hline
%Combined Context independent features & 0.63 & 0.83 & 0.62 & 0.72\\
%  \hline
%Combined Context dependent features & 0.52 & 0.92 & 0.52 &0.66\\
%\hline
%All features & 0.63 & 0.87 &  0.64 & 0.73\\
%\hline
%\end{tabular}
%%\vspace{-0.1in}
%\caption{Precision, recall, accuracy, and f-score for different features and feature sets on our test set (English only)}
%\label{FeatureEffectiveness}
%\vspace{-0.2in}
%\end{table*}
%
%\begin{table}[!th]
%\centering
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\textbf{Language} & \textbf{Precision} & \textbf{Recall} & \textbf{F-score} & \textbf{Accuracy}\\
%\hline
%English & 0.63 & 0.87 & 0.73 & 0.64\\
%\hline
%French & 0.59 & 0.86 & 0.70 & 0.6\\
% \hline
%German & 0.63 & 0.90 & 0.74 & 0.64\\
% \hline
%Spanish & 0.58 & 0.89 & 0.70 & 0.60\\
% \hline
%Japanese & 0.73 & 0.88 & 0.80 & 0.74\\
% \hline
% \end{tabular}
%% \vspace{-0.1in}
%\caption{Precision, recall, f-score and accuracy across various languages}
%\label{LanguagePerf}
%\vspace{-0.3in}
%\end{table}

%\begin{minipage}[b]{1\linewidth} 
%\centering
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\textbf{Algorithm} & \textbf{Precision} & \textbf{Recall} & \textbf{F-score} & \textbf{Accuracy}\\
%\hline
%Baseline Disambiguation and Linking algorithm & 0.55 & 0.99 & 0.7 & 0.62\\
%\hline
%Context-driven Entity Disambiguation and Linking algorithm  & 0.63 & 0.87 & 0.73 & 0.64\\
%\hline
%\end{tabular}
%\caption{Precision, Recall, F-score and Accuracy for our algorithm and baseline (English only)}
%\label{baselinecomparison}
%\end{minipage}
%\end{table*}

%\begin{figure}[t]
%  \centering
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=\textwidth,height=55mm]{figure/papyrus_performance_per_language_per_stage/eps/en_performance.eps}
%    \caption{Processing Stages for English}
%    \label{fig:processing_times_per_stage}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=\textwidth,height=55mm]{figure/papyrus_performance_per_language_per_stage/eps/ENTITY_DISAMBIGUATION_performance.eps}
%    \caption{Different Languages for Entity Disambiguation}
%    \label{fig:processing_times_per_language}
%  \end{subfigure}
%    \vspace{-0.1in}
%  \caption{Processing times as function of text length}
%  \label{fig:processing_times}
%  \vspace{-0.2in}
%\end{figure}

\subsection{Test datasets}
Using the process described in Section \ref{data_set}, we generated a ground truth test set of 20 English Wikipedia pages which had a total of 18,773 mentions. %We use this as our test set.

\subsection{Metrics}
We use standard performance metrics like precision, recall, f-score and accuracy to evaluate our NLP system components on the test sets. %However, due to our problem setup, we calculate true positives, false positives, and true negatives and false negatives in an unconventional way as shown in Table \ref{PositivesNegatives}. 
Precision, recall, f-score and accuracy are calculated as:
 $
 \textnormal{P} = {{\textnormal{$t_{p}$}} \over {\textnormal{$t_{p} $+ $f_{p}$}}}
$,
$
 \textnormal{R}= {{\textnormal{$t_{p}$}} \over {\textnormal{$t_{p}$ + $f_{n}$}}}
$,
$
 \textnormal{F1}= {{2 \times \textnormal{P} \times \textnormal{R}} \over {\textnormal{P + R}}}
$
and 
$
 \textnormal{Accuracy} = {{\textnormal{$t_{p}$ + $t_{n} $}} \over {\textnormal{$t_{p}$ + $t_{n}$ + $f_{p}$ + $f_{n}$}}}
$

\subsection{Results}\label{sec:results}
%Discussion about the features and results
%We compute the performance metrics for individual features as well as for various feature sets on our English language test set to assess their impact. % of individual features as well as feature sets. 
%Table \ref{FeatureEffectiveness} shows the feature effectiveness results for our algorithm. As evident from the results, \emph{Mention-Entity-Cooccurr} has the biggest impact on the performance of the algorithm among all individual features as it has the highest individual precision and f-score. %among all individual features. 
%
%When combined, the context independent features combined %(\emph{Mention-Entity-Cooccurr}, \emph{Mention-Entity-Jaccard} and \emph{Entity-Importance}) 
%have higher precision and f-score than the context dependent features. %(\emph{Entity-Entity-Cooccurr} and \emph{Entity-Entity-Topic-Sim}). 
%This could be due to the fact that in shorter text documents, there may not be enough easy mentions disambiguated in the first pass. 
%Since the context dependent features rely on the easy entity window for computation, their performance will be impacted. However, when all these features are taken together, the overall performance improves even further. This demonstrates that context is an important factor in entity disambiguation and linking.
%Our final algorithm, which utilizes all the context dependent and independent feature sets, has a precision of 63\%, recall of 87\% and f-score of 73\%. 
%
%Table \ref{LanguagePerf} shows the performance of the Lithium EDL system across various languages. We note that the test datasets for these languages are smaller. However, the algorithm's performance is comparable to that for the English dataset.

%\subsection{Comparison with baseline}
%We also compare our algorithm with a baseline algorithm that simply uses the most important context independent feature (\emph{Mention-Entity-Cooccurr}) score to disambiguate entities. Table \ref{baselinecomparison} shows the comparison of the two algorithms on the test data. The baseline algorithm has high Recall but low Precision.

\subsection{Runtime Performance}

The Lithium NLP system has been built to run in a bulk manner as well as a REST API service.
The two major challenges that we faced while developing the system were the volume of new data that we process in bulk daily and limited computational capacity. These challenges had a significant influence on our system design and algorithmic approach.

As a demonstrative example, the most consuming task in our MapReduce cluster processes around 910 million documents, with an average document size of 169 bytes, taking about 2.2ms per document. Our MapReduce cluster has around 150 Nodes each having a 2.5 GHz Xeon processor. The processing is distributed across 400 reducers. The Reduce step takes about 2.5 hrs. Each reducer task runs as a single thread with an upper bound of 7GB on memory where the processing pipeline and models utilize 3.7GB. 

A more detailed breakdown of the computational performance of our system as a function of document length is shown in Figure \ref{fig:processing_times}. The overall performance of the system is a linear function of text length. We also analyze this performance for different languages as well as for different stages of the Lithium NLP pipeline. 

%We can see that the computation is slowest for English since it has the maximum number of entities \cite{Spasojevic:dawt}.

% -- Some stats.
% CPU time spent (ms) 2,016,166,070
% Map output bytes	517,308,868,339	0	517,308,868,339
% Map output materialized bytes	153,880,824,483
% Map output records	908,428,345
% Reduce input groups	0	693,319,806	693319806
% Reduce input records	0	908428345	908428345
% Reduce output records	0	0	0
% Reduce shuffle bytes	0	153880824483	153880824483


==> texfiles/tuning.tex <==

%\begin{figure}
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=75mm ,height=60mm]{figures/FirstPassthresholdsPR.pdf}
%    \caption{Precision Recall curve for different values of first pass parameters $\lambda_{1}$ and $\lambda_{2}$}
%    \label{fig:firstpasspr}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=75mm ,height=60mm]{figures/WindowsizePR.pdf}
%    \caption{Precision Recall curve for different values of window size}
%    \label{fig:windowsizepr}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=75mm ,height=60mm]{figures/NoneMarginGainPR.pdf}
%    \caption{Precision Recall curve for different values of NONE margin gain}
%    \label{fig:nonemargingainpr}
%  \end{subfigure}
%  \label{Parameter Tuning Results}
%  \caption{Precision Recall curves for parameter tuning}
%\end{figure}


%We use part of our training data (generated as explained in Section \ref{data_set}) for tuning the hyper parameters. We split the data in a 7:3 ratio and use 70\% of the data for training. We use 20\% for testing and 10\% for validation.
Our algorithm uses four different hyperparameters - 2 in the first pass and 2 in the second pass. These are:

\begin{itemize}[noitemsep,nolistsep]
\item Easy mention disambiguation threshold with \textbf{NIL} ($\lambda_{1}$) - This threshold is used to disambiguate easy mentions which have 2 candidate entities and one of them is the \textbf{NIL} entity.
\item Easy mention disambiguation threshold ($\lambda_{2}$) - This threshold is used to disambiguate easy mentions which have 3 or more candidate entities but the mention maps to one of them with a very high prior probability.
%\end{itemize}

%The second pass parameters are:
%\begin{itemize}[noitemsep,nolistsep]
\item \textbf{NIL} margin of gain threshold ($\lambda_{3}$) - This threshold is used in the second pass to disambiguate entities when multiple or none of the candidates are labeled `True'.
\item Window size (\emph{W}) - This parameter represents the size of the easy entity window around each hard entity.
\end{itemize}

Using the process described in Section \ref{data_set}, we generated a ground truth validation set of 10 English Wikipedia pages which had a total of 7242 mentions and 23,961 candidate entities. We used parameter sweeping experiments to determine the optimal value of these parameters. We measured the performance (in terms of precision, recall and f-score) of the algorithm on the validation set with different parameter settings and picked the parameter values that had the best performance. 
%Figure \ref{fig:firstpasspr} shows the Precision-Recall curve for $\lambda_{1}$ $\in$ [0.85,0.95] and $\lambda_{2}$ $\in$ [0.75,0.95]. Figure \ref{fig:windowsizepr} shows the Precision-Recall curve for \emph{w} $\in$ [25,400]. Figure \ref{fig:nonemargingainpr} shows the Precision-Recall curve for $\lambda_{3}$ $\in$ [0.3,0.55].  
Based on our experiments, we set the optimal value of $\lambda_{1}$ as 0.75, $\lambda_{2}$ as 0.9, \emph{W} as 400 and $\lambda_{3}$ as 0.5. %as they achieve the highest Precision, Recall and F-score on the validation set.



